Software Between Quantum and Machine Learning -- And Down to Pulses

Contemporary quantum computing platforms remain, in essence, programmable physical systems whose control is typically mediated through unitary gate abstractions. While such abstractions provide a uniform interface, they obscure important aspects of the underlying hardware and may limit the exploitation of its full capabilities. Direct operation at the control-pulse level offers a more expressive and physically faithful paradigm, enabling, for instance, the implementation of tailored error-mitigation and optimisation strategies. However, this increased expressivity comes at the cost of greater quantum software development complexity, necessitating structured and accessible tooling. We present a software framework, integrated within the QML-Essentials package, that extends quantum machine learning (QML) methodologies to encompass pulse-level modelling. By embedding quantum optimal control techniques within a QML setting, our approach enables the seamless combination of gate-based and pulse-level representations. The framework provides a comprehensive suite of modelling and analytical capabilities. In particular, we introduce composable ansatz constructions based on interchangeable building blocks, and support for end-to-end optimisation of pulse parameters. Motivated by the central role of quantum Fourier models, we further incorporate a range of Fourier-analytic diagnostics, complemented by extended measures of entanglement. All performance-critical components are implemented in a high-performance environment using JAX and supported by a dedicated quantum simulator. Taken together, the framework facilitates reproducible and systematic investigations, while bridging the conceptual and practical divide between abstract circuit models and hardware-aware optimisation. It provides a robust foundation for future developments at the intersection of QML and quantum control.

==> tikz-figs/code_snippets/ansatzlist.tex <==
\begin{python}
"Hardware_Efficient", "Strongly_Entangling",
"Circuit_1", "Circuit_2", ...
\end{python}


==> tikz-figs/code_snippets/execution.tex <==
\begin{python}[emphstyle=\ttb\color{execution_col}]
out = m(
  inputs=x,
  params=p,
  pulse_params=pp
)
\end{python}


==> tikz-figs/code_snippets/metrics.tex <==
\begin{python}[emphstyle=\ttb\color{metrics_col}]
coeffs, freqs = Coefficients.get_spectrum(m)
fcc = FCC.get_fcc(m)

inv_expr = Expressibility.kl_divergence_to_Haar(m)

ent_cap = Entanglement.meyer_wallach(m)
\end{python}


==> tikz-figs/code_snippets/model.tex <==
\begin{python}[emphstyle=\ttb\color{model_col}]
m = Model(
    n_qubits=4,
    n_layers=1,
    circuit_type="Strongly_Entangling",
    initialization="random",
    data_reuploading=True,
)
\end{python}


==> tikz-figs/code_snippets/topology.tex <==
\begin{python}[aboveskip=-5pt, belowskip=-4pt, basicstyle=\ttmsmall]
stairs, brick,
all_to_all
\end{python}

